Dependent Session Types

Session types offer a type-based discipline for enforcing communication protocols in distributed programming. We have previously formalized simple session types in the setting of multi-threaded $\lambda$-calculus with linear types. In this work, we build upon our earlier work by presenting a form of dependent session types (of DML-style). The type system we formulate provides linearity and duality guarantees with no need for any runtime checks or special encodings. Our formulation of dependent session types is the first of its kind, and it is particularly suitable for practical implementation. As an example, we describe one implementation written in ATS that compiles to an Erlang/Elixir back-end.

==> before.tex <==



\newcommand{\Lzero}[0]{\mathcal{L}_0}
\newcommand{\Ldep}[0]{\mathcal{L}_{\forall,\exists}}
\newcommand{\Lchan}[0]{\mathcal{L}_{\forall,\exists}^{\pi}}


\def\ATS{$\mathcal{A}\mathcal{T}\kern-.1em\mathcal{S}$}
\def\res{\mathcal{R}}

% utility
\newcommand{\defeq}[0]{\coloncolonequals}
\newcommand{\dom}[0]{\text{\rm\bf dom}}

% syntax
\newcommand{\sort}[1]{\text{\rm\it #1}}
\newcommand{\type}[1]{\text{\rm\bf #1}}
\newcommand{\stype}[1]{\text{\rm\tt #1}}
\newcommand{\subtype}[0]{\leq_{ty}}
\newcommand{\sta}[1]{\text{\rm\it #1}}
\newcommand{\dyn}[1]{\text{\rm\bf #1}}
\newcommand{\guard}[0]{\,{\supset}\,}
\newcommand{\guardi}[0]{{\supset^+}}
\newcommand{\guarde}[0]{{\supset^-}}
\newcommand{\foralli}[0]{\forall^+}
\newcommand{\foralle}[0]{\forall^-}
\newcommand{\assert}[0]{{\wedge}}

% common constants
\newcommand{\sig}[0]{\mathcal{S}}
\newcommand{\dcx}[0]{\textit{dcx}}
\newcommand{\dcc}[0]{\textit{dcc}}
\newcommand{\dcf}[0]{\textit{dcf}}
\newcommand{\dcr}[0]{\textit{dcr}}
\newcommand{\scx}[0]{\textit{scx}}
\newcommand{\scc}[0]{\textit{scc}}
\newcommand{\scf}[0]{\textit{scf}}

\newcommand{\chan}[0]{\type{chan}}
\newcommand{\msg}[0]{\stype{msg}}
\newcommand{\quan}[0]{\stype{quan}}
\newcommand{\fix}[0]{\stype{fix}}
\newcommand{\nil}[0]{\stype{end}}
\newcommand{\branch}[0]{\stype{branch}}
\newcommand{\ite}[0]{\stype{ite}}


% shirk figures
% \setlength{\abovecaptionskip}{-1ex}

\newcommand{\cli}[0]{\stype{C}}
\newcommand{\srv}[0]{\stype{S}}

% for pushing floats to the top instead of scraching them on the whole page

\makeatletter
\setlength{\@fptop}{0pt}
\setlength{\@fpsep}{\floatsep}
\setlength{\@fpbot}{0pt plus 1fil}
\makeatother

==> header.tex <==


\usepackage{colonequals} % for ::= and ::
\usepackage[a]{esvect} % for \vv
\usepackage{prftree}
\usepackage{adjustbox} % for stackbox

% amsthm is preloaded with the template
\newtheorem{prop}[theorem]{Proposition}


\usepackage[capitalise,noabbrev,nameinlink]{cleveref} % for \cref
\crefname{lemma}{Lemma}{Lemmas}
\crefname{ex}{Example}{Examples}
\crefname{app}{Appendix}{Appendix}


\usepackage{pgfmath}
\usepackage{tikz}
\usetikzlibrary{arrows,shapes,petri}

==> mtlc0evalctx.tex <==
\begin{align*}
\text{evaluation context}~E \defeq~& [] \mid \dcx\,(\vv{v}, E, \vv{e}) \mid \langle E,e\rangle \mid \langle v,E\rangle \mid 
                                     \dyn{let}~\langle x_1,x_2\rangle=E~\dyn{in}~e \mid\\
                                   & \dyn{if}~E~\dyn{then}~e_1~\dyn{else}~e_2 \mid \dyn{fst}(E) \mid \dyn{snd}(E) \mid \dyn{app}(E,e) \mid \dyn{app}(v,E)
\end{align*}

==> session.tex <==



\begin{figure}[p]
\caption{Examples}
\begin{align*}
\stype{counter} &\defeq \stype{fix}(\lambda f{:}(\sort{int}\rightarrow\sort{stype}).\lambda n{:}\sort{int}.\stype{branch}(1, \stype{msg}(0, \type{int}(n)) \coloncolon f(n+1), \stype{end}(1))) \\
\stype{counter} (n{:}\sort{int}) &\defeq \stype{branch}(1, \stype{msg}(0, \type{int}(n)) \coloncolon \stype{counter}(n+1), \stype{end}(1)) \\
\stype{repeat}  (a{:}\sort{vtype}, n{:}\sort{int}) &\defeq \stype{ite}(n>0, \stype{msg}(1, a) \coloncolon \stype{repeat}(a,n-1), \stype{end}(1)) \\
\stype{array}   (a{:}\sort{vtype}) &\defeq \quan(1, \lambda n{:}\sort{int}.\stype{msg}(1, \type{int}(n))::\stype{repeat}(a, n))
\end{align*}
\end{figure}

==> syntax.tex <==









\begin{figure}[!p]
\caption{Types}
\[
\begin{array}{rrcl}
\text{types}   \quad & \tau     & \defeq & a \mid \delta(\vv{s}) \mid \type{1} \mid \tau_1 \times \tau_2 \mid \tau_1 \rightarrow \tau_2 \mid P\guard\tau \mid P\assert\tau \mid \forall a {:} \sigma. \tau \mid \exists a {:} \sigma.\tau            \\
\text{vtypes}  \quad & \hat\tau & \defeq & \hat{a}\mid\hat\delta(\vv{s}) \mid \tau \mid \hat\tau_1\otimes\hat\tau_2 \mid \hat\tau_1\multimap\hat\tau_2 \mid   P\guard\hat\tau \mid P\assert\hat\tau \mid \forall a{:}\sigma.\hat\tau \mid \exists a{:}\sigma.\hat\tau \\
\text{stypes}  \quad & \pi      & \defeq & \stype{end}(\sort{int}) \mid \stype{msg}(\sort{int}, \hat\tau) \coloncolon \pi \mid \stype{branch}(\sort{int}, \pi_1, \pi_2) 
\end{array}
\]
\end{figure}


\begin{figure}[!p]
\caption{Some Static Constants}
\[
\begin{array}{rclrcl}
\
\times & : & (\sort{type}, \sort{type})   \Rightarrow \sort{type}     & \otimes & : & (\sort{vtype}, \sort{vtype}) \Rightarrow \sort{vtype}    \\
\rightarrow & : & (\sort{type}, \sort{type}) \Rightarrow \sort{type} & \multimap & : & (\sort{vtype}, \sort{vtype}) \Rightarrow \sort{vtype} \\
\guard & : & (\sort{bool}, \sort{type}) \Rightarrow \sort{type} & \guard & : & (\sort{bool}, \sort{vtype}) \Rightarrow \sort{vtype} \\
\assert & : & (\sort{bool}, \sort{type}) \Rightarrow \sort{type} & \assert & : & (\sort{bool}, \sort{vtype}) \Rightarrow \sort{vtype} \\
\forall & : & (\sigma \rightarrow \sort{type}) \Rightarrow \sort{type} & \forall & : & (\sigma \rightarrow \sort{vtype}) \Rightarrow \sort{vtype} \\
\exists & : & (\sigma \rightarrow \sort{type}) \Rightarrow \sort{type} & \exists & : & (\sigma \rightarrow \sort{vtype}) \Rightarrow \sort{vtype} \\
\type{int}  & : & () \Rightarrow \sort{type} & \type{int}  & : & (\sort{int}) \Rightarrow \sort{type} \\
\type{bool}  & : & () \Rightarrow \sort{type} & \type{bool}  & : & (\sort{bool}) \Rightarrow \sort{type} \\
\stype{end} & : & (\sort{int}) \Rightarrow \sort{stype} & \stype{msg} & : & (\sort{int}, \sort{vtype}, \sort{stype}) \Rightarrow \sort{stype} \\
\stype{branch} & : & (\sort{int}, \sort{stype}, \sort{stype}) \Rightarrow \sort{stype} \\
\type{chan} & : & (\sort{stype}) \Rightarrow \sort{vtype} \\
\subtype & : & (\sort{type}, \sort{type}) \Rightarrow \sort{bool}
\end{array}
\]
\end{figure}


\begin{figure}[!p]
\caption{Dynamic Language Syntax}
\[
\begin{array}{rrcl}
\text{dynamic constant}      \quad & \textit{dcx} & \defeq & \textit{dcc} \mid \textit{dcf}                                                                        \\
\text{dynamic terms}         \quad & e            & \defeq & x \mid \textit{dcx}\,(\vv{e}) \mid \textit{dcr} \mid \langle \rangle \mid \langle e_1, e_2 \rangle \mid \\
													&&& \dyn{fst}(e) \mid \dyn{snd}(e) \mid \dyn{lam}~x.e \mid \dyn{app}(e_1, e_2) \mid                      \\
               										&&& \guardi(v) \mid \guarde(e) \mid  \assert(e) \mid \dyn{let}~{\assert}(x)=e_1~\dyn{in}~e_2~\dyn{end} \mid                              \\
               										&&& \foralli(v) \mid \foralle(e)  \mid \exists(e) \mid \dyn{let}~\exists(x)=e_1~\dyn{in}~e_2~\dyn{end}                                   \\
\text{dynamic values}        \quad & v            & \defeq & x \mid \textit{dcx}\,(\vv{v}) \mid \langle\rangle \mid \langle v_1,v_2 \rangle \mid \dyn{lam}~x.e \mid \guardi(v) \mid \foralli(v) \mid \assert(v) \mid \exists(v)         								  \\

\text{dynamic type context}  \quad & \Gamma       & \defeq & \varnothing \mid \Gamma, x : \tau                                                         \\
\text{dynamic vtype context} \quad & \Delta       & \defeq & \varnothing \mid \Delta, \hat{x} : \hat\tau                                               \\
\text{dynamic signature}     \quad & \mathcal{S}  & \defeq & \varnothing \mid \mathcal{S}, \textit{dcx}: (\vv{\tau}) \Rightarrow \tau \mid \mathcal{S}, \textit{dcx}: (\vv{\hat\tau}) \Rightarrow \hat\tau \\
\text{dynamic substitutions} \quad & \theta       & \defeq & [] \mid \theta[x \mapsto v] \\
\text{pools}				 \quad & \Pi          & \defeq & [] \mid \Pi[t \mapsto e] \\
\end{array}
\]
\end{figure}


